Towards Understanding Cyberbullying Behavior in a Semi-Anonymous Social Network

Cyberbullying has emerged as an important and growing social problem, wherein people use online social networks and mobile phones to bully victims with offensive text, images, audio and video on a 247 basis. This paper studies negative user behavior in the Ask.fm social network, a popular new site that has led to many cases of cyberbullying, some leading to suicidal behavior.We examine the occurrence of negative words in Ask.fms question+answer profiles along with the social network of likes of questions+answers. We also examine properties of users with cutting behavior in this social network.

==> ctype.tex <==
% !TEX root = ICWSM_paper.tex
\section{Cyberbullying Types}

We were also interested in understanding whether different types of cyberbullying could be discerned from our data. Cyberbullying manifests itself in a variety of different forms, including racial, religious, sexual and appearance-based cyberbullying.  Figure \ref{fat1} shows an example of appearance-based cyberbullying that we've observed.  Recall that this words graph has been built with our initial 1500 negative words set. Based on our initial analysis, we believe that groups of words tend to be used together for certain types of cyberbullying, and that these word groups may be sufficiently distinctive to be used as a basis for identifying some kinds of cyberbullying. Our thinking was to develop word graph models that are representative for each kind of cyberbullying.\comment{, and then match an individual profile’s word graph to the models.}


\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.3\textwidth]{./fig/muslim1}  % use this if you use "pdflatex"
\caption{An observation on occurrence of religious cyberbullying in Ask.fm, visualized using Gephi \cite{Gephi}.}
\label{muslim1} % Fig.3
\end{figure} 


\begin{figure}[htb!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.3\textwidth]{./fig/fat1}  % use this if you use "pdflatex"
\includegraphics[width=0.4\textwidth]{./fig/apearance_fat_ugly}
\caption{An observation on occurrence of appearance cyberbullying in Ask.fm, visualized using Gephi \cite{Gephi}.}
\label{fat1} % Fig.3
\end{figure}

Towards this end, we constructed word graph models centered around certain types of bullying words.  For example, Figure  \ref{muslim1} illustrates a word graph clustered around the word ``muslim", which is associated with religious cyberbullying, while Figure \ref{fat1} illustrate a word graph based around the ``fat", which is associated with appearance-based cyberbullying.  Words with higher eigenvector centrality are shown with larger diameters.  We observe that the two graphs exhibit clearly distinct patterns that differ in the number of words associated with the core word, which words are clustered around the core word, and the strength of association between the words and the core word.

Another way to visualize the differences between religious, appearance-based, sexual (LBGT) and racial  cyberbullying is to analyze the distribution of negative words associated with each type of cyberbullying.
For this purpose we first find all profiles with a specific word among the 27.9K gathered profiles, then for those profiles find the distribution of the 80 negative words of our reduced collection and compute an average over them. Figure \ref{fat_dist} shows the frequency of negative words seen with the word ``fat", while Figure \ref{muslim_dist} plots the frequency of negative words seen with the word ``muslim".  The top 80 negative words are constant across the x-axis of both graphs. We see that the word ``muslim" is used with words in the 0-10 and 40-50 ranges that do not show up for ``fat"-based cyberbullying.

Even within a category of cyberbullying, there can be distinctions.  For example, in sexually-based LGBT cyberbullying, Figure \ref{LGB} shows the frequency of negative words for three separate words: ``lesbian", ``bisexual" and ``gay".  We observe that the distributions are distinguishable both in terms of the presence/absence of peaks at specific word IDs, and also in terms of the height of peaks.  In particular, the word ``lesbian" has strong peaks of association with the words ``ugly" and ``f**k" that are absent or only half as strong as for sexual cyberbullying using the word ``gay".  Also, even though the ``fat"-based distribution's shape resembles the ``lesbian"-based distribution, the distinction is that the peaks of the former are half the frequency values of the latter.

On the other hand, Figure \ref{racial} reveals that there is a similar pattern of distribution of negative words based around the words ``black" and ``asian" for racial cyberbullying.  Overall, the most distinctive pattern appears to be ``muslim"-based religious cyberbullying.

\comment{
Distribution of negative words around words: muslim, fat, bisexual, gay, lesbian, black, asian as potential subjects prone to different cyberbullying types shown in figure \ref{fat_dist}-\ref{racial}. We can see in Figure \ref{LGB} the frequency of negative words around word lesbian is bigger than bisexual and gay. Also word lesbian has its highest value around word ``ugly" and then the f-word. For word gay the highest frequency word is the f-word which is approximately half of the value seen for lesbian. In fact, looking at \ref{fat_dist} subject fat has a histogram similar to lesbian, with smaller frequency. We can see the word ``muslim'' has been seen with the words:  ``d**ck, f**k, hate''.

On the other hand, subjects gay, black and bisexual receive negative words with the same pattern. Subject muslim has the most distinguishable frequency over negative words. 


Figure \ref{racial} shows two subject ``black" and ``asian" receive approximately the same frequency of negative words.
}

%Such a graph would measure how groups of negative words are used together in a profile’s discussion. For example, we illustrate a contextual  word graph built from the word relationships, and highlight the connections with the word "gay" in Figure \ref{figgay}. In contrast, we see a word graph that highlights connections between words and the
%word "black" in Figure \ref{figblack}. We observe that the sets of words most strongly connected with "gay"and "black" appear to be different. We can use these word graphs to discern patterns and to derive key properties. For example, we have found that there are much fewer negative words grouped around the word "lesbian" than the word "gay" (latter is used in more hate speech). Also, we have observed that the word "cut" has been connected to the word "depress". This association could be used to detect vulnerable victims of cyberbullying. We can see the word ``muslims'' has been seen with the words:  ``disgusting, hate, bomb, bloody, racist''.

 %Appearance cyberbullying has been observed looking at this network, as for example the word ``fat'' has been seen with the huge set of negative words, like ``ugly, die, stupid, shit, slut,...''. In this project we skip considering different type of bullying and just stick with the general case of victim versus normal users. By looking at the words with highest Eigenvector centrality a set of 100 words has been collected. Table shows the 17 words with highest frequency and eigen vector centrality obtained from the words network has been shown. 




\begin{figure}[!ht]
\begin{minipage}[b]{0.48\linewidth}
\centering
\includegraphics[width=\textwidth]{./fig/fat3-eps-converted-to.pdf}
\caption{Frequency of negative words seen with the word ``fat" as an example of appearance-based cyberbullying}
\label{fat_dist}
\end{minipage}
%\hspace{0.5cm}
\hfill
\begin{minipage}[b]{0.48\linewidth}
\centering
\includegraphics[width=\textwidth]{./fig/mslm3-eps-converted-to.pdf}
\caption{Frequency of negative words seen with the word ``muslim" as an example of religious cyberbullying}
\label{muslim_dist}
\end{minipage}
\end{figure}
%\begin{figure}[!ht]
%\begin{minipage}[b]{0.48\linewidth}
%\centering
%\includegraphics[width=\textwidth]{./fig/gay.pdf}
%\caption{Frequency of negative words seen with word gay as an example of LGB cyberbullying}
%\label{gay}
%\end{minipage}
%\hspace{0.5cm}
%\hfill
%\begin{minipage}[b]{0.48\linewidth}
%\centering
%\includegraphics[width=\textwidth]{./fig/les.pdf}
%\caption{Frequency of negative words seen with word lesbian as an example of LGB cyberbullying}
%\label{les}
%\end{minipage}
%\end{figure}
%\begin{figure}[!ht]
%\begin{minipage}[b]{0.48\linewidth}
%\centering
%\includegraphics[width=\textwidth]{./fig/black.pdf}
%\caption{Frequency of negative words seen with word black as an example of racial cyberbullying}
%\label{black}
%\end{minipage}
%\hspace{0.5cm}
%\hfill
%\begin{minipage}[b]{0.48\linewidth}
%\centering
%\includegraphics[width=\textwidth]{./fig/bi.pdf}
%\caption{Frequency of negative words seen with word bisexual as an example of LGB cyberbullying}
%\label{bi}
%\end{minipage}
%\end{figure}

\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.5\textwidth]{./fig/LGB-eps-converted-to.pdf}  % use this if you use "pdflatex"
\caption{Frequency of negative words seen with words ``lesbian", ``bisexual", ``gay" as an example of LGB cyberbullying}
\label{LGB} % Fig.3
\end{figure} 

\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.5\textwidth]{./fig/rcial-eps-converted-to.pdf}  % use this if you use "pdflatex"
\caption{Frequency of negative words seen with words ``black" and ``asian" as an example of racial cyberbullying}
\label{racial} % Fig.3
\end{figure} 

\subsection{High Risk Cyberbullying}
One of the most disturbing behaviors that we encountered was the problem of ``cutting" (slicing one's wrists).  In these cases, it seemed that the victims were particularly vulnerable to bullies, and exhibited weak confidence and depression problems, sometimes admitting to earlier failed attempts at suicide.  We term such users as being at high risk of the consequences of cyberbullying.  In this section we first find all the profiles for which their owners have expressed the experience of ``cutting" behavior. We observe in Figure \ref{cut1} that among the words that the word ``cut" has been connected to are the words ``depress", ``stressful", ``sad", and ``suicide" . This association could be used to detect vulnerable victims of cyberbullying. 

\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.3\textwidth]{./fig/cut1}  % use this if you use "pdflatex"
\caption{An observation on occurrence of high risk cyberbullying in Ask.fm, visualized using Gephi \cite{Gephi}.}
\label{cut1} % Fig.3
\end{figure} 

The frequency of negative words used with ``cut" has been shown in Figure \ref{ct}. We can see these user profiles also have two peaks at words ``ugly" and ``f**k" similar to appearance-based and LGBT-based cyberbullying.
 
\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.5\textwidth]{./fig/cut2-eps-converted-to.pdf}  % use this if you use "pdflatex"
\caption{Frequency of negative words seen with word "cut".}
\label{ct} % Fig.3
\end{figure}


\begin{table}[htb]
\centering
\begin{tabular}{|c|c|}
\hline 
Average number of questions per user  &  	 15	\\ \hline
Average number of negative questions per user 	  & 2.3125\\ \hline
Average number of positive questions per user   &    5.2891\\ \hline
Average number of negative words per user 	  & 3.3750\\ \hline
Average number of positive words per user   & 6.6484\\ \hline
\end{tabular}
\caption{Average number of questions and words per user with ``cutting" label}
\label{stats_cut}
\end{table} 

Table  \ref{stats_cut} illustrates the statistics of those users for which the word ``cut" appeared in their profiles.  Comparing Table \ref{stats2} with Table \ref{stats_cut}, we see that high risk profiles in average have 1.2 times less negative questions with 1.4 less negative words per question compare to labeled victim profiles. Also they have 1.23 times more positive questions than victim profiles. This suggests surprisingly but encouragingly that high risk profiles do receive more support and less bullying posts compared to general cyberbullying victims. 

Table \ref{highrisk} shows the statistics of the average reciprocity, in-degree and out-degree for high risk victims.  They appear to exhibit collectively a different behavior than HN, HP, PN, OTHR and even generally labeled victims.  This deserves further investigation to explain the reasons behind the differences.

\begin{table}[htbp]\centering
\begin{tabular}{lclclclclclcl} %\hline
                        & 	Labeled high risk victims \\ \hline
Negative reciprocity     &  	 0.1463  \\
Non-Negative reciprocity	 &   0.2481\\ %\hline
Negative in-degree	     & 	17.8790 \\ %\hline
non-Negative in-degree	 &  78.7177 \\ %\hline
Negative out-degree      & 	 4.4194 \\ %\hline
non-Negative out-degree	 &  64.9758 \\ %\hline
\end{tabular}
\caption{Average reciprocity and degree for high risk victims}
\label{highrisk}
\end{table}   

==> netstat.rick.tex <==
% !TEX root = ICWSM_paper.tex
\section{Network statistics}

\subsection{Building the interaction graph}

\comment{As there is no friendship which connect to user, in fact two users are connected if there is an interaction between them. The only non-anonymous interaction among users is liking the question/answer in each other pages.}  

Though we had collected 150K profiles, our original method was limited in that it could only retrieve the first page of likes, not the complete list of users who liked a question/answer.  To obtain a more complete picture of the liking behavior, we collected and analyzed  27910 profiles that had a complete list of likes.  As mentioned, we focused on the top 15 most liked questions.  We found that there were on average 14.4723 most liked questions per user, that is most users had close to 15 questions with likes.  We also focused on a collection of 80 negative words and 80 positive words with the highest eigenvector centrality as explained in previous section.


\begin{table}[htb]
\centering
\begin{tabular}{|c|c|}
\hline 
Questions per user  &  	 14.4723	\\ \hline
negative questions per user 	  & 0.7776\\ \hline
positive questions per user   &    4.5733\\ \hline
negative words per user 	  & 1.0394\\ \hline
positive words per user   & 5.4196\\ \hline
\end{tabular}
\caption{Average number of questions and words per user}
\label{stats}
\end{table}




Out of 27910 profiles, 12845 users or 46.02\% have at least one question including one of the top negative words. We term such a question a ``negative" question.  Furthermore, 2159 users or 7.74\% of the users have at least three questions with top negative words. 26779 or 95.95\% users had at least question with a top positive word in their profiles. We term such a question a "positive" question.  Table ~\ref{stats} shows the average number of positive and negative questions and words per user.

Next, by a one mode projection of the bipartite graph, we were able to obtain the like-based interaction graph U between these 27910 users in the Ask.fm social network.  We restricted our analysis to consider likes for only the top 15 most liked questions/answers on each user profile.  In the adjacency matrix U, created from the users' interaction graph, edges are weighted. In fact the weight of each edge $e_{ij}$ , from node $i$ to node $j$ is a vector $w_{ij}=[n_1 n_2]$, where $n_1$ is the number of questions in node $j$ including at least one negative word (from our selected dictionary) and $n_2$ is the number of questions with no negative word liked by node $i$. Since we are most interested in negative behavior, we group positive and neutral behavior together into a "non-negative" category. 

For further analysis, we have divided matrix U into two matrices UN and Un-N. In fact UN  (Negative adjacency matrix) is the adjacency matrix with weights $n_1$ and An-N (non-Negative adjacency matrix) is the adjacency matrix with weights $n_2$. 

Figure \ref{figDist} shows the CCDF for the in-degree and out-degree distribution of matrices UN and Un-N. Authors in \cite{Mislove} show that in-degree and out-degree distributions in social networks are approximately  the same. We can see from Figure \ref{figDist} the in-degree and out-degree for non-negative degree distribution is approximately the same for non-negative degree distributions, however it is a little different for negative degree distributions, which indicates that negative behavior has different properties than previously reported for normal behavior.

\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.35\textwidth]{./fig/out_in_neg_lil.pdf}  % use this if you use "pdflatex"
\caption{CCDF for negative and non-negative interaction graphs/matrices.}
\label{figDist} % Fig.3
\end{figure} 



The mean reciprocity of the interaction graph/matrix U is 28.20\%, which is a low number compare to other social networks like Yahoo! 360 with reciprocity 84\% and Flickr with reciprocity 68\%. However twitter has a more similar structure to Ask.fm (in the sense that there is no friendship concept between users) and has an even lower reciprocity equal to 22.1\%.
The network negative reciprocity is a very low 3.61\%, which shows how much negative questions of each other users like. In fact it gives an insight that users who both have negative posts do not tend to like each others' negative questions. Reciprocity between non-negative questions is 27.94\%, which is 12 times higher. 

\begin{figure}[!ht]
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=\textwidth]{./fig/non_neg_rcp_lil.pdf}
%\caption{Typical public profile on Ask.fm with questions/comments (usually anonymous) to the profile owner and answers from the profile owner.}
\label{fig:mobile1}
\end{minipage}
\hspace{0.15cm}
\begin{minipage}[b]{0.45\linewidth}
\centering
\includegraphics[width=\textwidth]{./fig/neg_rcp_lil.pdf}
%\caption{An example of anonymous cyberbullying comments posted on a user's profile in Ask.fm.}
\label{fig:mobile2}
\end{minipage}
\caption{Reciprocity for non-negative and negative interaction graphs/matrices}
\label{fig:recip}
\end{figure}

Figure \ref{fig:recip} shows the mean reciprocity for the two graphs/matrices UN and Un-N versus out-degree. It shows that in normal (non-negative) behavior the more active a user is, the more he/she will receive likes from other users or vice versa. On the other hand, the mean reciprocity increases much slower in the negative matrix. When the negative out-degree is high, this means that a user is active and likes others user's negative questions\comment{(we do not know for sure as support or to bully them)}. However he/she does receive few negative in-degree comments in return. Again, we see that negative behavior follows a different pattern than non-negative behavior.

To relate the preceding graph analysis to cyberbullying, we obtained ground truth for cyberbullying by
labeling a set of 150 profiles as examples of cyberbullying. Users of this labeled data set have a minimum of 1 and a maximum of 8 negative questions. The average number of negative questions is 2.8716.  They have in average 4.3333 positive questions, which implies they have support on their wall beside the negative posts.  Table \ref{stats2} summarizes these results.  We see compared to Table \ref{stats} that the pattern of negative questions is quite different.


\begin{table}[htb]
\centering
\begin{tabular}{|c|c|}
\hline 
Questions per user  &  	 14.8718 \\ \hline
negative questions per user 	  & 2.8716\\ \hline
positive questions per user   &    4.3333\\ \hline
negative words per user 	  & 4.7179\\ \hline
positive words per user   & 6.0769 \\ \hline
\end{tabular}
\caption{Average number of questions and words per labeled victim of cyberbullying}
\label{stats2}
\end{table}



%why in-degree on negative questions is small even when the out-degree is high?  

 \comment{It shows that person is either supportive and popular- probably dos not receive that much negative questions- or is bully and unpopular, and even if has negative questions, dos not receive likes. }

By looking at the content of these cyberbullying profiles, we see that they have on average about 3 negative questions, so we chose a threshold of 3 negative questions to define a group that we term Highly Negative (HN). In fact, we segmented the user base into 4 different groups:\\
 
\begin{enumerate}
\item	Highly Negative: users with at least 3 negative posts and no positive posts (HN)
\item	Highly Positive: users with more than 10 positive posts (HP)
\item	Positive-Negative: users with at least 3 negative posts and more than 4 positive posts (PN)
\item	Others (OTR)
\end{enumerate}

The definition of these groups helps us identify the properties of the most vulnerable victims of cyberbullying, namely the HN users who have no positive support, while also allowing us to contrast them with the graph properties of other users who have some or a lot of positive words in support.  Figure \ref{figRec} shows an example of a mixed profile with both positive and negative comments, representative of the PN group.

\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.35\textwidth]{./fig/negativ_positive1}  % use this if you use "pdflatex"
\caption{An example of a profile with both positive and negative comments.}
\label{figRec} % Fig.3
\end{figure} 


\comment{
In fact group 1 and group 2 both are affected by cyberbullying, as they have at least three negative questions and it will be count as a repeated behavior. Also we are not claiming that group 1 and 3 cover all cyberbullying case. Group 4 can also have victims. The goal of separating to these groups is looking closely at users with some similar statistics and evaluating their other features. We observed that victims could be divided in a group who receive support from bystanders and a group who have been left alone and don?t receive any support, and therefore we get the idea of considering group 1 and 2. Now we look at the reciprocity of each group we defined earlier.
}


\begin{table*}[htbp]\centering
\begin{tabular}{lclclclclclcl} %\hline
tab                        & HN        & 	HP	     & PN	     &     OTHR   & 	Labeled victims \\ \hline
Negative reciprocity     &  0.1310     &   	0     &  0.1056    &  0.0655  &	0.0987 \\
Non-Negative reciprocity	 & 0.2100     &  0.3792    &  0.2464    &  0.3391  & 	0.2729 \\ %\hline
Negative in-degree	     & 6.3864     &     0     & 13.9935    &  2.1614   & 	6.33 \\ %\hline
non-Negative in-degree	 & 21.0909    & 111.7111  & 49.4478    &  70.0660	  & 26.8 \\ %\hline
Negative out-degree      & 	3.4773    & 2.7345    &  3.7293    &  3.5870   & 	2.359 \\ %\hline
non-Negative out-degree	 & 32.7955    & 116.7618  & 45.9717    & 70.0512	  & 23.52 \\ %\hline
\end{tabular}
\caption{Average reciprocity and degree for different groups}
\end{table*} 

Table \ref{table:keyresults} summarizes some of the key results of our graph analysis.  We measure the average reciprocity of the four different groups, as well as the in-degree and out-degree.  We further separate the in-degree into two subcategories, pertaining to negative in-degree and non-negative in-degree, i.e. a user X will have a negative in-degree if another user likes one of the questions posted on X's profile that has a negative word in it, while another user liking a question without a negative word will count towards the non-negative in-degree of X.  Similarly, we divide out-degree into negative and non-negative subcategories.

HN users have the smallest in-degree and the smallest out-degree. It shows they are either not popular or do not tend to have activity in this social network. However, when we look at negative out-degree, HP users have the smallest out-degree, which shows they are the most active group. It means HP users not only do not have negative posts, but also do not like negative posts or do not have that much friends with negative posts. 

	Negative in-degree of the group PN is more than twice of group HN. The mean number of negative questions for group HN is 3.72 and for group PN is 3.73, which approximately the same as at the first place we assigned the same limitation on number of negative questions for both of these groups. On the other hand, the average number of positive questions in HN and PN group are respectively 0.7636 and 6.5244, while each group have in average the total number of questions 14.7 and 15 respectively. Therefore, we can conclude the in-degree on negative questions (likes on negative questions) is a sign of support, as we observed PN group has more support than HN group on receiving positive posts on their wall. As we said, there is only one button for question and answer. Looking at some profiles, gave us the insight that likes are mostly representative of support and a positive sign. Observing that PN groups have negative in-degree 2 times bigger than HN groups agrees with our assumption. 
Looking at negative reciprocity, it is obvious that HP has negative reciprocity 0 as it dos not have any negative in-degree. In the group OTHR there exist either a set of users with 1 or 2 negative questions without any limitation on the positive posts, or a set of users with more than 2 negative questions and less than 10 positive questions. However, the average number of negative questions is 0.7737, which shows we have mostly users belong to first set. We see that the reciprocity on negative questions in this group is lower than HN and PN groups. The reason is either because they have few negative questions compare to HN and HP groups (which in average the have less), or they have less support (they have in average 4.7 positive questions compared to 6.5 positive questions for HP group).  

\comment{
To relate the preceding graph analysis to cyberbullying, we obtained ground truth for cyberbullying by
labeling a set of 150 profiles as examples of cyberbullying. Users of this labeled data set have a minimum of 1 and a maximum of 8 negative questions. The average number of negative questions is 2.8716, which is close to HN and HP group. They have in average 4.3333 positive questions, which implies they have mostly support on their wall beside the negative posts, table \ref{stats2}. Their out-degree is pretty low, even lower than HN, which show low out degree is a good indicator of cyberbullying. The negative in-degree is smaller than HP group?s and bigger HN group's. However, we expect a bigger number compare the average of positive questions that they have received in their pages. In general we can say this set of label data has pretty low in-degree and out-degree.
}



In order to calculate the local clustering coefficient for each node we first turned our network to a simple graph. It means either node i has liked node j?s question, or node j has liked node i?s question, regardless of how many times, we set $U_{ij} = 1$ and $U_{ji} = 1$, otherwise $U_{ij} = U_{ji} = 0$. We make this assumption that either user i receives a like from user j or posts a like on his/her profile, they are in the general category of having some familiarity or ``connectedness''. The expected clustering coefficient of the network is 0.1095 using formula 7.41 and the averaged local clustering coefficient 0.3564 using formula 7.44 of the book \cite{netbook}. Comparing with numbers reported by \cite{data}, shown in table 3 the clustering coefficient is pretty small. In Figure \ref{LCC} the local clustering as a function of degree has been depicted. As we expect local clustering coefficient decrease when the degree increase in social networks. 

\begin{table*}[htbp]\centering
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline 
social media & ``Ask.fm'' & 	Facebook & Twitter & 	Gplus & 	Orkut & Flicker & Orkut & You Tube  \\ \hline
Clustering Coefficient & 	0.3564 & 	0.6055	 & 0.5653 & 	0.4901	 & 0.1666 & 0.313 & 0.171 & 0.136 \\ \hline 
%Clustering Coefficient & 	0.1095 & 	0.2647 & 	0.06415 & 	0.6552 & 	0.01414\\ \hline 
\end{tabular}
\caption{Local clustering coefficient for some social networks}
\label{LLC_web}
\end{table*}



Looking at the clustering coefficient of each group, we observe that among 4 defined groups, HN with the lowest degree has highest mean local clustering coefficient and group HP with highest degree has the lowest mean local clustering. The implication is that users of HN group probably have a few friends that they know each other. However, users of HP group are very social and they know lots of people, and therefore the ratio of their friends that they know each other is small. In general, we can see each group that has higher degree has lower mean local clustering.  However, for the labeled victims we can see the mean local clustering is smaller than HN, although its out degree is smaller than HN group.

\begin{table}[htb]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
	HN & 	HP	 & PN & 	OTHR	 & Labeled victims\\ \hline
 	0.4986    &  	0.2365   &   	0.3798    &  	0.3573	 & 0.4096\\ \hline

\end{tabular}
\caption{Local clustering coefficient for defined group}
\label{tab:weblog-data}
\end{table}


\begin{figure}[htbp!]\centering
%\psfig{file=rosette.ps, height=1in, width=1in}
\includegraphics[width=0.35\textwidth]{./fig/MLCCvsK-eps-converted-to.pdf}  % use this if you use "pdflatex"
\caption{Mean local clustering coefficient versus degree}
\label{LCC} % Fig.3
\end{figure} 


